Bayesian and Frequentist Semantics for Common Variations of Differential Privacy: Applications to the 2020 Census

The purpose of this paper is to guide interpretation of the semantic privacy guarantees for some of the major variations of differential privacy, which include pure, approximate, R\'enyi, zero-concentrated, and $f$ differential privacy. We interpret privacy-loss accounting parameters, frequentist semantics, and Bayesian semantics (including new results). The driving application is the interpretation of the confidentiality protections for the 2020 Census Public Law 94-171 Redistricting Data Summary File released August 12, 2021, which, for the first time, were produced with formal privacy guarantees.

==> composition.tex <==
\subsubsection{Composition}
\textcolor{red}{Please do not edit the file composition.tex. I will be editing if offline and uploading to overleaf}
\pbdp also has fully adaptive composition properties. Here we present a result that shows the composition is sub-additive.

\begin{theoremEnd}[category=privdefs]{theorem}\label{thm:pbdpfullcomp}
Let $\mech_1,\dots, \mech_k$ be a sequence of mechanisms with the following properties:
\begin{itemize}
\item The input to $\mech_1$ is the data $\data$ and privacy parameters $\epsilon_1,\delta_1$.  For any fixed $\epsilon_1,\delta_1$, $\mech_1$ satisfies $(\epsilon_1,\delta_1)$-\pbdp when viewed as a function of $\data$. The output of $\mech_1$ is denoted $(\outp_1,\epsilon_2,\delta_2)$. Here $\epsilon_2$ and $\delta_2$ are interpreted to be privacy parameters for $\mech_2$.
\item For $i=2,\dots, k$, the input to $\mech_i$ consists of (1) $\data$, (2) the  $\outp_{i-1}$ produced by $\mech_{i-1}$, (3) the parameters $\epsilon_i,\delta_i$ produced by $\mech_i$. For any fixed $(\outp_{i-1},\epsilon_i,\delta_i)$, $\mech_i$ satisfies $(\epsilon_i,\delta_i)$-\pbdp when viewed as a function of $\data$. The output of $\mech_i$ is denoted $(\outp_i,\epsilon_{1+1},\delta_{i+1})$. If $i\neq k$ then $\epsilon_{1+1}$ and $\delta_{i+1}$ are interpreted to be privacy parameters for the next mechanism.  
\item The internal randomness of every mechanism is independent of its input and of the internal randomness of the other mechanisms.
\end{itemize}
Furthermore, suppose that for some $\epsilon$ and $\delta$, $\sum_{i=1}^k \epsilon_i\leq\epsilon$ and $\sum_{i=1}^k \delta_i\leq\delta$ with probability 1. Then $\mech^*$ that runs these mechanisms in a sequence and outputs the result of $\mech_k$ satisfies $(\epsilon,\delta)$-\pbdp.
\end{theoremEnd}

\begin{proofEnd}[proof here]
We will be using Theorem \ref{thm:pbdpequiv} Item \ref{item:pbdp3}.	
	
Let $\randalg^*$ be a postprocessing function whose domain contains the range of $\mech^*$ and whose output is either 0 or 1. 

Define the sequence of random variables $(X^{\outp}_1, Y^\epsilon_1, Z^\delta_1),\dots, (X^{\outp}_k, Y^\epsilon_k, Z^\delta_k)$  so that $(X^{\outp}_i, Y^\epsilon_i, Z^\delta_i)$ represents the $(\outp_i,\epsilon_{i+1},\delta_{i+1})$ output by $\mech_i$ when the underlying dataset is $\data_1$. So that this notation also covers $\mech_k$, we set $Y^\epsilon_{k}=\perp$ and $Z^\delta_{k}=\perp$ (since the last mechanism does not output privacy parameters), and for convenience, $X^{\outp}_0=\perp$, $Y^\epsilon_0=\epsilon_1$ and $Z^\delta_0=\delta_1$ (so $Y^\epsilon_0$ and $Z^\delta_0$ are the privacy parameters fed into $\mech_1$). Note that $(X^{\outp}_1, Y^\epsilon_1, Z^\delta_1),\dots, (X^{\outp}_k, Y^\epsilon_k, Z^\delta_k)$  are correlated since, for example, $(X^{\outp}_i, Y^\epsilon_i, Z^\delta_i)$ is fed into $\mech_{i+1}$ (or into $\randalg^*$ when $i=k$) along with the specific dataset $\data_1$ to produce $(X^{\outp}_{i+1}, Y^\epsilon_{i+1}, Z^\delta_{i+1})$. Thus the joint distribution of $(X^{\outp}_1, Y^\epsilon_1, Z^\delta_1),\dots, (X^{\outp}_k, Y^\epsilon_k, Z^\delta_k)$ is the same as the joint distribution of the intermediate results in the execution of $\mech^*$ and this is important because it means $\sum_{i=0}^{k-1} Z^\delta_i\leq\delta$ and $\sum_{i=0}^{k-1} Y^\epsilon_i\leq\epsilon$ with probability 1.

Now define the following mechanisms $B_1,\dots, B_k$ with randomness independent of each other and independent of $\mech^*$. The input to $B_i$ is similar to $\mech_i$: it gets a dataset $\data$, an auxiliary input $\outp^b$, and privacy parameters $\epsilon^b$ and $\delta^b$. $B_i(\data,\outp^b,\epsilon^b, \delta^b)$ first runs $\mech_i(\data, \outp^b,\epsilon^b, \delta^b)$ and then feeds its output, along with the specific dataset $\data_2$ in $\mech_{i+1}$, then feeds that output along with $\data_2$ into $\mech_{i+1}$, etc. and then runs $\randalg^*$ at the end. Note that $\mech_i$ is the only one of these that gets $\data$ as input, the subsequent mechanisms only get the fixed dataset $\data_2$ as input and hence are part of a long postprocessing phase. Thus $B_i$ satisfies $(\epsilon^b,\delta^b)$-\pbdp for each choice of $\outp^b,\epsilon^b$, and $\delta^b$ since $\mech_i$ does. 

We note the following facts that are true by construction:
\begin{itemize}
	\item The output distribution of $\mech^*(\data_1)$ is identical to that of  $B_k(\data_1, X^{\outp}_{k-1}, Y^\epsilon_{k-1}, Z^\delta_{k-1})$.
	\item The output distribution of $\mech^*(\data_2)$ is identical to that of $B_1(\data_2, X^{\outp}_{0}, Y^\epsilon_{0}, Z^\delta_{0})$
	\item The output distribution of $B_i(\data_1, X^{\outp}_{i-1}, Y^\epsilon_{i-1}, Z^\delta_{i-1})$ is identical to that of $B_{i+1}(\data_2), X^{\outp}_i, Y^\epsilon_i, Z^\delta_i)$.
	\item If $\log\frac{P(\randalg^*(\mech^*(\data_1))=1)}{P(\randalg^*(\mech^*(\data_2))=1)}>\epsilon$ then $\log\frac{P(\randalg^*(\mech^*(\data_1))=1)}{P(\randalg^*(\mech^*(\data_2))=1)}>\log\frac{P(\randalg^*(\mech^*(\data_1))=0)}{P(\randalg^*(\mech^*(\data_2))=0)}$ (since the output of $\randalg^*\circ\mech^*$ is either 0 or 1) and this further implies that $P(\plrv[\data_1][\data_2][\mech^*]>\epsilon)=P(\randalg^*(\mech^*(\data_1))=1)$.
\end{itemize}
Using these facts, we note that for $x\in\{0,1\}$,
\begin{align*}
\log\frac{P(\randalg^*(\mech^*(\data_1))=x)}{P(\randalg^*(\mech^*(\data_2))=x)} &=  \sum_{i=1}^k  \frac{P(B_i(\data_1, X^{\outp}_{i-1}, Y^\epsilon_{i-1}, Z^\delta_{i-1})=x)}{P(B_i(\data_2, X^{\outp}_{i-1}, Y^\epsilon_{i-1}, Z^\delta_{i-1})=x)} 
\end{align*}
and so $\log\frac{P(\randalg^*(\mech^*(\data_1))=1)}{P(\randalg^*(\mech^*(\data_2))=1)} > \epsilon$ means that for at least one $i$, we have

Consider the random variable $\plrv[\data_1][\data_2][\randalg^*\circ\mech^*]=\log\frac{P(\randalg^*(\mech^*(\data_1))=x)}{P(\randalg^*(\mech^*(\data_2))=x)}$ where $x$ is sampled from the output distribution of $\randalg^*(\mech^*(\data_1))$. 

Without loss of generality, we may assume $P(\randalg^*(\mech^*(\data_1))=1)> e^\epsilon P(\randalg^*(\mech^*(\data_2))=1)$ (otherwise the conditions of the theorem trivially hold for this choice of $\randalg^*$) and this means  $\frac{P(\randalg^*(\mech^*(\data_1))=0)}{P(\randalg^*(\mech^*(\data_1))=0)} < 1$. Thus $P(\plrv[\data_1][\data_2][\randalg^*\circ\mech^*] > e^\epsilon) = P(\randalg^*(\mech^*(\data_1))=1)$ and our goal is to show that this is $\leq \delta$.

Now define the algorithm $B_i$ as follows. $B_i(\data)$ chains together $\mech_1,\dots, \mech_k$ similarly to $\mech^*$. However, for $j=1,\dots, i-1$ it feeds $\data_1$ into $\mech_j$, it feeds $\data$ into $\mech_i$, and for $j=i+1,\dots, k$ it feeds $\data_2$ into $\mech$. Notice that $B_k(\data_1)$ is probabilistically the same as $\mech^*(\data_1)$, $B_1(\data_2)$ is probabilistiically the same as $\mech^*(\data_2)$, and $B_i(\data_1)$ is probabilistically the same as $B_{i+1}(\data_2)$ for $i=1,\dots, k-1$.
Thus,
\begin{align*}
\log\frac{P(\randalg^*(\mech^*(\data_1))=x)}{P(\randalg^*(\mech^*(\data_2))=x)} &= \sum_{i=1}^k \log\frac{P(B_i(\data_1)=x)}{P(B_i(\data_2)=x)}
\end{align*}

and so $\plrv[\data_1][\data_2][\randalg^*\circ\mech^*]$ is the sum of $k$ correlated random variables $X_1,\dots, X_k$, where the marginal distribution of $X_i$ is that 

\end{proofEnd}

Note that in Theorem \ref{thm:pbdpfullcomp}, each mechanism $\mech_i$ can include in the variable $\outp_i$ the outputs of all of the previous mechanisms, thus, we lose no generality by only assuming the output of $\mech_k$ is released.

Theorem \ref{thm:pbdpfullcomp} only takes advantage of one setting of $(\epsilon_i,\delta_i)$ for each mechanism $\mech_i$. Better composition results are possible if more information is known about each mechanism. These results leverage privacy accounting performed by zcdp and rdp, which we discuss in Section \ref{sec:rzcdp}. 


\begin{comment}

\pbdp has naive composition results analogous to approximate differential privacy.

\begin{textAtEnd}[category=privdefs,both]
We now need the following result that lets us switch between the  $\plrv[\data_1][\data_2][\mech]$ and its reversed variable $\plrv[\data_2][\data_1][\mech]$.
\end{textAtEnd}
\begin{theoremEnd}[category=privdefs]{lemma}\label{lem:change}
For any $\mech$, $\data_1,\data_2$ and $s\leq t$, 
$$e^{s}P(\plrv[\data_2][\data_1][\mech] \in [-t, -s]) \leq P(\plrv[\data_1][\data_2][\mech]\in [s, t]) \leq e^t P(\plrv[\data_2][\data_1][\mech] \in [-t, -s])$$
Furthermore, if $s_1\leq t_1\leq s_2\leq t_2$ then
$$\frac{P(\plrv[\data_1][\data_2][\mech_1]\in [s_1,t_1])}{P(\plrv[\data_2][\data_1][\mech_1]\in [-t_1, -s_1])} \leq \frac{P(\plrv[\data_1][\data_2][\mech_1]\in [s_2,t_2])}{P(\plrv[\data_2][\data_1][\mech_1]\in [-t_2, -s_2])}$$
whenever the denominators are nonzero (and analogous results hold for open and semi-open intervals like $(s_1, t_1]$), and finally, both $\frac{P(\plrv[\data_1][\data_2][\mech_1]\geq s)}{P(\plrv[\data_2][\data_1][\mech_1]\leq -s)}$ and $\frac{P(\plrv[\data_1][\data_2][\mech_1]> s)}{P(\plrv[\data_2][\data_1][\mech_1]< -s)}$ are nondecreasing functions of $s$ whenever the denominators are nonzero.
\end{theoremEnd}
\begin{proofEnd}[proof here]
We prove this in the discrete case. For the continuous case, replace the probability mass functions with the density functions.
Let $S_{[s,t]}=\{\omega~:~\log \frac{P(\mech(\data_1)=\omega)}{P(\mech(\data_2)=\omega)} \in [s,t]\}$. Then by definition of the privacy loss random variable, 
\begin{align*}
P(\plrv[\data_1][\data_2][\mech]\in [s, t]) &= P(\mech(\data_1) \in S_{[s, t]})\\
P(\plrv[\data_2][\data_1][\mech]\in [-t, -s]) &= P(\mech(\data_2)\in S_{[s,t]})
\end{align*}
By definition of $S_{[s,t]}$ it easily follows that
$$e^{s}P(\mech(\data_2) \in S_{[s, t]}) \leq P(\mech(\data_1) \in S_{[s, t]}) \leq e^t P(\mech(\data_2) \in S_{[s, t]})$$
and the first result follows. Then using this result, we see that when the denominators are not 0,
$$\frac{P(\plrv[\data_1][\data_2][\mech_1]\in [s_1,t_1])}{P(\plrv[\data_2][\data_1][\mech_1]\in [-t_1, -s_1])} \leq e^{t_1}\leq e^{s_2} \leq \frac{P(\plrv[\data_1][\data_2][\mech_1]\in [s_2,t_2])}{P(\plrv[\data_2][\data_1][\mech_1]\in [-t_2, -s_2])}$$
from which the second result follows. Finally, for $s_1\leq s_2$, when none of the following have zero denominators,
\begin{align*}
\frac{P(\plrv[\data_1][\data_2][\mech_1]\geq s_1)}{P(\plrv[\data_2][\data_1][\mech_1]\leq -s_1)} &= 
\frac{P(\plrv[\data_1][\data_2][\mech_1]\in[s_1, s_2)) + P(\plrv[\data_1][\data_2][\mech_1]\geq s_2)}{P(\plrv[\data_2][\data_1][\mech_1]\in (-s_2. -s_1]) + P(\plrv[\data_2][\data_1][\mech_1]\leq -s_2)}\\
&\leq \max\left(\frac{P(\plrv[\data_1][\data_2][\mech_1]\in[s_1, s_2))}{P(\plrv[\data_2][\data_1][\mech_1]\in (-s_2. -s_1])},
\frac{ P(\plrv[\data_1][\data_2][\mech_1]\geq s_2)}{ P(\plrv[\data_2][\data_1][\mech_1]\leq -s_2)}
\right) = \frac{ P(\plrv[\data_1][\data_2][\mech_1]\geq s_2)}{ P(\plrv[\data_2][\data_1][\mech_1]\leq -s_2)}
\end{align*}
where the last equality follows from the second result.
\end{proofEnd}


\begin{theoremEnd}[category=privdefs]{theorem}\label{thm:pbdpcomp}
Let $\mech_1$ and $\mech_2$ be two mechanisms that satisfy \pbdp with parameters $(\epsilon_1,\delta_1)$ and $(\epsilon_2,\delta_2)$, respectively. The mechanism that, on input $\data$, releases both $\mech_1(\data)$ and $\mech_2(\data)$ satisfies $(\epsilon_1+\epsilon_2, \delta_1+\delta_2)$-\pbdp.
\end{theoremEnd}
\begin{proofEnd}[proof here]
Our proof leverages Definition \ref{def:pbdp} directly.

Pick a pair of neighbors $\data_1,\data_2$. We will use $\data$ (without subscripts) as a variable to denote a dataset in general (it may be $\data_1$ or $\data_2$ or some other dataset).

Now let $\mech^*$ be the mechanism that, on input $\data$, releases $(\mech_1(\data), ~\mech_2(\data))$ and let $\randalg^*$ be any (possibly randomized) algorithm that postprocesses the output of $\mech^*$. We will use $\randalg^*$ to define a postprocessing algorithm $\randalg_1$ for the output of $\mech_1$ and also a postprocessing algorithm $\randalg_2$ for the output of $\mech_2$. 

Define $\randalg_1$ so that $\randalg_1(\mech_1(\data))= \randalg^*(\mech_1(\data), \mech_2(\data_2))$. That is, for any arbitrary $\data$, $\randalg_1$ takes $\mech_1(\data)$, runs $\data_2$ through $\mech_2$, and releases $\randalg^*$ applied to the pair of outputs. Note that $\randalg_1$ is properly a postprocessing function -- anyone who has $\mech_1(\data)$ can run $\randalg_1$ since it uses no other information about the true data (i.e., the extra randomness it introduces is the same, no matter what $\data$ is, and hence is independent of the true data).

Similarly define $\randalg_2$ so that $\randalg_2(\mech_2(\data)) = \randalg^*(\mech_1(\data_1), \mech_2(\data))$. That is, $\randalg_2$ takes its input $\mech_2(\data)$, computes $\mech_1(\data_1)$ and feads both of those outputs into $\randalg^*$. Similarly to $\randalg_1$, running $\randalg_2$ does not require any knowledge of the true data beyond $\mech_2(\data)$.

Now, $\plrv[\data_1][\data_2][\randalg^*\circ\mech^*]$ has the distribution of $\log\frac{P(\randalg^*(\mech_1(\data_1), \mech_2(\data_1))=\omega)}{P(\randalg^*(\mech_1(\data_2), \mech_2(\data_2))=\omega}$ when $\omega$  is sampled from the output distribution of $\randalg^*(\mech_1(\data_1), \mech_2(\data_1))$. This is the same as the distribution of 
$$\log\frac{P(\randalg^*(\mech_1(\data_1), \mech_2(\data_1))=\omega)}{P(\randalg^*(\mech_1(\data_1), \mech_2(\data_2))=\omega)}
+
\log\frac{P(\randalg^*(\mech_1(\data_1), \mech_2(\data_2))=\omega)}{P(\randalg^*(\mech_1(\data_2), \mech_2(\data_2))=\omega)}$$ when when $\omega$  is sampled from the output distribution of $\randalg^*(\mech_1(\data_1), \mech_2(\data_1))$.

For $\mech_1$, choose the smallest  $\tau_1$ and associated $c_1\in[0,1]$,  such that 
$c_1 P(\plrv[\data_1][\data_2][\mech_1]>\tau_1)+ (1-c_1) P(\plrv[\data_1][\data_2][\mech_1]\geq \tau_1) 
= \delta_1$. Similarly, for $\mech_2$ choose the smallest $\tau_2$ and associated $c_2\in [0,1]$ such that $c_2 P(\plrv[\data_1][\data_2][\mech_2]>\tau_2)+ (1-c_2) P(\plrv[\data_1][\data_2][\mech_2]\geq \tau_2) 
= \delta_2$. Note that since $\delta_1$ and $\delta_2$ are in $[0,1]$  then $\tau_1,\tau_2,c_1,c_2$ are guaranteed to exist (but $\tau_1$ and $\tau_2$ may be $\pm\infty$).

First, we can rule out some easy cases:
\begin{itemize}
\item If $\tau_1=-\infty$ then $\delta_1=1$ and clearly the result holds. Similarly if $\tau_2=-\infty$ then the result is trivial.
\item If $\epsilon_1=\infty$   or $\epsilon_2=\infty$ then everything is vacuous.
\item $\tau_1=\infty$ or $\tau_2=\infty$ mean either $\epsilon_1=\infty$ or $\epsilon_2=\infty$ and reverts back to the previous case.
\item If $\plrv[\data_1][\data_2][\mech_1]\leq \epsilon_1$ with probability 1 \textbf{and} $\plrv[\data_1][\data_2][\mech_2]\leq \epsilon_2$ with probability 1, then again the result is trivial since the privacy loss random variable $\plrv[\data_1][\data_2][\mech^*]\leq \epsilon_1+\epsilon_2$ with probability 1.
\end{itemize}
and so without loss of generality, we can assume that the $\epsilon$ and $\tau$ values are all finite.

\textbf{Next we consider the case where
  $\plrv[\data_1][\data_2][\mech_1]\leq \epsilon_1$ with probability 1 but $\plrv[\data_1][\data_2][\mech_2]$ is not bounded by $\epsilon_2$}. In this case,  $\delta_1=0$. Consider the threshold $\tau^*=\epsilon_1+\tau_2$ and $c^*=c_2$. Then $\plrv[\data_1][\data_2][\mech^*]> \epsilon_1+\tau_2$ implies that $\plrv[\data_1][\data_2][\mech_2]> \tau_2$ and  $\plrv[\data_1][\data_2][\mech^*]\geq \epsilon_1+\tau_2$ implies that $\plrv[\data_1][\data_2][\mech_2]\geq \tau_2$.
This means $c_2P(\plrv[\data_1][\data_2][\mech^*]> \epsilon_1+\tau_2) + (1-c_2)P(\plrv[\data_1][\data_2][\mech^*]\geq \epsilon_1+\tau_2) \leq c_2P(\plrv[\data_1][\data_2][\mech_2]> \tau_2) + (1-c_2)P(\plrv[\data_1][\data_2][\mech_2]\geq \tau_2)\leq \delta_2=\delta_1+\delta_2$. Furthermore 
 (for the continuous case, replace with densities and integration)
\begin{align*}
\lefteqn{\frac{c_2P(\plrv[\data_1][\data_2][\mech^*] > \epsilon_1+\tau_2) + (1-c_2)P(\plrv[\data_1][\data_2][\mech^*] \geq \epsilon_1+\tau_2)}
{c_2 P(\plrv[\data_2][\data_1][\mech^*] < -(\epsilon_1+\tau_2)) + (1-c_2)P(\plrv[\data_2][\data_1][\mech^*] \leq -(\epsilon_1+\tau_2))}}\\
%
&=\frac{ \sum_s P(\plrv[\data_1][\data_2][\mech_1] = s) \left(c_2P(\plrv[\data_1][\data_2][\mech_2] > \tau_2 + (\epsilon_1-s)) + (1-c_2)P(\plrv[\data_1][\data_2][\mech_2] \geq \tau_2 + (\epsilon_1-s))\right)} %end top of frac
{\sum_s P(\plrv[\data_2][\data_1][\mech_1] =-s)\left( c_2P(\plrv[\data_2][\data_1][\mech_2] < -\tau_2 - (\epsilon_1-s)) + (1-c_2)P(\plrv[\data_2][\data_1][\mech_2] \leq -\tau_2-(\epsilon_1-s))\right)}\\
%
&\phantom{=}\text{by choice of $\tau_2$, }
\end{align*}


So, we can assume that $\tau_1>-\infty$, $\tau_2>-\infty$, $\epsilon_1<\infty$, $\epsilon_2<\infty$.

We first consider the case where  $\delta_1>0$ and $\delta_2>0$.


Let $S^1_{(>\tau_2)}$ be the set of possible outputs of $\mech_1$ that satisfy $\{\omega~:~\log\frac{P(\mech_1(\data_1)=\omega)}{P(\mech_1(\data_2)=\omega)} > \tau_1\}$, let $S^2_{(>\tau_1)}$ be the set possible outputs of $\mech_2$ that satisfy $\{\omega~:~\log\frac{P(\mech_2(\data_1)=\omega)}{P(\mech_2(\data_2)=\omega)} > \tau_2\}$. Define $S^1_{(\geq\tau_1)}$ and $S^2_{(\geq\tau_2)}$ analogously.

Note that by the definition of privacy loss random variable, we have, for example, $ P(\plrv[\data_1][\data_2][\mech_1]>\tau_1) = P(\mech_1(\data_1)\in S^1_{(>\tau_1)})$ and this means: $c_1 P(\mech_1(\data_1)\in S^1_{(>\tau_1)}) + (1-c_1) P(\mech_1(\data_1)\in S^1_{(\geq\tau_1)})=\delta_1$ and $c_2 P(\mech_2(\data_1)\in S^2_{(>\tau_2)}) + (1-c_2) P(\mech_2(\data_1)\in S^2_{(\geq\tau_2)})=\delta_2$. 

To simplify the argument, for every $\omega_1\in S^1_{(\geq\tau_1)}\setminus S^1_{(>\tau_1)}$ we will replace it with 2 items  called $\omega_1^{in}$ that has $(1-c_1)$ times the mass of $\omega_1$ and $\omega_1^{out}$ that has $c_1$ times the mass of $\omega_1$. Without loss of generality, we will assume that $\mech_1$ outputs one of these instead of $\omega_1$ (i.e., if $\mech_1$ wants to output some $\omega_1\in S^1_{(\geq\tau_1)}\setminus S^1_{(>\tau_1)}$ then with probability $1-c$ it will attach the ``in" superscript to $\omega_1$ and otherwise it will attach the ``out'' superscript). We do the same with $\omega_2\in S^2_{(\geq\tau_2)}\setminus S^2_{(>\tau_2)}$, so that we get a 
$\omega_2^{in}$ that has $(1-c_2)$ times the mass of $\omega_2$ and $\omega_2^{out}$ that has $c_2$ times the mass of $\omega_2$.

This means we can define the set $B_1$ to be the union of $S^1_{(>t)}$ and all the elements of $S^1_{(\geq\tau_1)}\setminus S^1_{(>\tau_1)}$ that have an ``in'' superscript. This means that all of the following are true:
\begin{itemize}
\item[(i)] $P(\mech_1(\data_1)\in B_1) = c_1 P(\mech_1(\data_1)\in S^1_{(>\tau_1)}) + (1-c_1) P(\mech_1(\data_1)\in S^1_{(\geq\tau_1)})=\delta_1$
\item[(ii)] If $\omega\in B_1$ and $\omega^\prime\notin B_1$ then $\log\frac{P(\mech_1(\data_1)=\omega)}{P(\mech_1(\data_2)=\omega)}\geq \log\frac{P(\mech_1(\data_1)=\omega^\prime)}{P(\mech_1(\data_2)=\omega^\prime)}$
\item[(iii)] If $S\subset B_1$ and $S^\prime\subset \overline{B}_1$ (the complement of $B_1$) and if $P(\mech_1(\data_1)\in S)=P(\mech_1(\data_1)\in S^\prime)$ then $P(\mech_1(\data_2)\in S) \leq P(\mech_1(\data_2)\in S^\prime)$. In other words, if $S$ and $S^\prime$ have the same probability when $\data_1$ is the input, $S$ cannot have larger probability than $S^\prime$ when $\data_2$ is the input.
\end{itemize}
Note that $B_1$ was defined for mechanism $\mech_1$ and we can analogously define $B_2$ for mechanism $\mech_2$ with analogous properties to those above.

Now consider the set $B^*= \{(\omega_1,\omega_2)~:~\omega_1\in B_1 \text{ or }\omega_2\in B_2\}$ which captures a subset of possible outputs of $\mech^*$. We see that:
\begin{align}
P(\mech^*(\data_1)\in B^*)&\leq P(\mech_1(\data_1)\in B_1) + P(\mech_2(\data_1)\in B_2) = \delta_1+\delta_2\\
%
%
\log\frac{P(\mech^*(\data_1)\in B^*)}{P(\mech^*(\data_2)\in B^*)} 
%
&\leq\log\frac{P(\mech_1(\data_1)\in B_1)P(\mech_2(\data_1)\in B_2) }
{P(\mech_1(\data_2)\in B_1)P(\mech_2(\data_2)\in B_2)}\leq\epsilon_1+\epsilon_2\label{eqn:the_two_eps}
\end{align}
where the first inequality in Equation \ref{eqn:the_two_eps} comes from the fact that $B^*$ is the disjoint union  $B_1\times \overline{B}_2 \cup\overline{B}_1\times B_2 \cup B_1\times B_2$. Of the three sets that make up the union, $B_1\times B_2$ has the largest probability ratio for $\mech^*$ under $\data_1$ compared to $\data_2$. This follows from property (ii) of $B_1$ above (and the corresponding property for $B_2$) and Lemma \ref{lem:change}.
Note that the first inequality in Equation \ref{eqn:the_two_eps} assumes that both $B_1$ and $B_2$ are nonempty, which is guaranteed when $\delta_1>0$ and $\delta_2>0$.

Now choose sets $S_a$, $S_b$  and $\lambda\in[0,1]$ such that 
$P(\mech^*(\data_1)\in S_a) + \lambda P(\mech^*(\data_1)\in S_b)=\delta_1+\delta_2$.
We want to show that
$\log\frac{P(\mech^*(\data_1)\in B^*)}{P(\mech^*(\data_2)\in B^*)}\geq \frac{P(\mech^*(\data_1)\in S_a) + \lambda P(\mech^*(\data_1)\in S_b}{P(\mech^*(\data_2)\in S_a) + \lambda P(\mech^*(\data_2)\in S_b}$, which would complete the proof for the $\delta_1>0, \delta_2>0$ case in light of Equation \ref{eqn:the_two_eps} and Theorem \ref{thm:pbdpequiv}. To simplify the discussion, we again replace items in $S_b$ with an ``in'' version that has $\lambda$ of the mass and an ``out'' version that has $1-\lambda$ of the mass, and define $S^*$ to be the set that is equal to $S_a$ and all the ``in'' items of $S_b$. Then $P(\mech^*(\data_1)\in S^*)=\delta$ and our goal is to prove that $\log\frac{P(\mech^*(\data_1)\in B^*)}{P(\mech^*(\data_2)\in B^*)}\geq \frac{P(\mech^*(\data_1)\in S^*)}{P(\mech^*(\data_2)\in S^*)}$.


%If $\delta_1=0$ it follows directly from the definition that these two complementary privacy loss random variables satisfy $\plrv[\data_1][\data_2][\mech_1]\leq \epsilon_1$ and
%$\plrv[\data_2][\data_1][\mech_1]\geq -\epsilon_1$.
%Therefore the following two complementary privacy loss random variables satisfy:
%\begin{align*}
%\plrv[\data_1][\data_2][\mech^*] &= \plrv[\data_1][\data_2][\mech_2] + \plrv[\data_1][\data_2][\mech_1] \leq \plrv[\data_1][\data_2][\mech_2] + \epsilon_1\\
%
%\plrv[\data_2][\data_1][\mech^*] &= \plrv[\data_2][\data_1][\mech_2] + \plrv[\data_2][\data_1][\mech_1] \geq \plrv[\data_2][\data_1][\mech_2] - \epsilon_1\\
%\end{align*}
%and so for any $\tau$,
%\begin{align*}
%P(\plrv[\data_1][\data_2][\mech^*] > \tau) &\leq P(\plrv[\data_1][\data_2][\mech_2] > \tau -\epsilon_1) \\
%P(\plrv[\data_2][\data_1][\mech^*] < -\tau) &\geq %P(\plrv[\data_2][\data_1][\mech_2] < -(\tau -\epsilon_1))
%\end{align*}

%with probability 1. \textcolor{red}{todo}
We first consider the case where $\delta_1=0$. Note that for any $\tau$,
\begin{align*}
%\lefteqn{
%c(P(\plrv[\data_1][\data_2][\mech^*] > \tau) - e^{\epsilon_1+\epsilon_2}P(\plrv[\data_2][\data_1][\mech^*]) <-\tau) + (1-c)(P(\plrv[\data_1][\data_2][\mech^*] \geq \tau) - e^{\epsilon_1+\epsilon_2}P(\plrv[\data_2][\data_1][\mech^*]) \geq -\tau)}
%\\
\lefteqn{ P(\plrv[\data_1][\data_2][\mech^*] > \tau) - e^{\epsilon_1+\epsilon_2}P(\plrv[\data_2][\data_1][\mech^*] < -\tau)} \\
%
&= \sum_{s\leq \epsilon_1} P(\plrv[\data_1][\data_2][\mech_2] > \tau-s )P(\plrv[\data_1][\data_2][\mech_1] = s)  -e^{\epsilon_1+\epsilon_2} 
\sum_{s\leq \epsilon_1} P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-s) )P(\plrv[\data_2][\data_1][\mech_1] = -s)  \\
%
%
&= \sum_{s\leq \epsilon_1} P(\plrv[\data_1][\data_2][\mech_2] > \tau-s )P(\plrv[\data_1][\data_2][\mech_1] = s)  -e^{\epsilon_1+\epsilon_2} 
\sum_{s\leq \epsilon_1} P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-s) )e^{-s}P(\plrv[\data_1][\data_2][\mech_1] = s)\\
&\text{ by Lemma \ref{lem:change}}  \\
%
%
&= \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] > \tau-s )   
-e^{\epsilon_1+\epsilon_2-s}P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-s) )
\right)P(\plrv[\data_1][\data_2][\mech_1] = s) \\
%
%
&\leq \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] > \tau-s )   
-e^{\epsilon_2}P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-s) )
\right)P(\plrv[\data_1][\data_2][\mech_1] = s) \\
&\text{ since $s\leq \epsilon_1$ with probability 1}
%
%
%&= \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] > \tau-\epsilon_1 )   
%-e^{\epsilon_1+\epsilon_2-s}P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-\epsilon_1) )
%\right)P(\plrv[\data_1][\data_2][\mech_1] = s)  \\
%
%&\phantom{ = }-
% \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] \in (\tau-\epsilon_1, \tau-s] )   
%-e^{\epsilon_1+\epsilon_2-s}P(\plrv[\data_2][\data_1][\mech_2] \in [-(\tau-s), -(\tau-\epsilon_1)) )
%\right)P(\plrv[\data_1][\data_2][\mech_1] = s) \\ 
%
%
%&\leq \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] > \tau-\epsilon_1 )   
%-e^{\epsilon_1+\epsilon_2-s}P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-\epsilon_1) )
%\right)P(\plrv[\data_1][\data_2][\mech_1] = s)  \\
%
%&\phantom{ = }-
%\sum_{s\leq \epsilon_1} \left( e^{\tau-\epsilon}P(\plrv[\data_2][\data_1][\mech_2] \in [-(\tau-s), -(\tau-\epsilon_1)))   
%-e^{\epsilon_1+\epsilon_2-s}P(\plrv[\data_2][\data_1][\mech_2] \in [-(\tau-s), -(\tau-\epsilon_1)) )
%\right)P(\plrv[\data_1][\data_2][\mech_1] = s)  \\
%&\text{By Lemma \ref{lem:change}}\\
%
%
%&\leq \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] > \tau-\epsilon_1 )   
%-e^{\epsilon_1+\epsilon_2-s}P(\plrv[\data_2][\data_1][\mech_2] < -(\tau-\epsilon_1) )
%\right)P(\plrv[\data_1][\data_2][\mech_1] = s)  \\
%
%&\phantom{ = }-
%\sum_{s\leq \epsilon_1} \left( e^{\tau-\epsilon}  
%-e^{\epsilon_1+\epsilon_2-s}\right)P(\plrv[\data_2][\data_1][\mech_2] \in [-(\tau-s), -(\tau-\epsilon_1)) )
%P(\plrv[\data_1][\data_2][\mech_1] = s)  
\end{align*}
and similarly,
$$P(\plrv[\data_1][\data_2][\mech^*] \geq \tau) - e^{\epsilon_1+\epsilon_2}P(\plrv[\data_2][\data_1][\mech^*] \leq -\tau)\leq \sum_{s\leq \epsilon_1} \left(P(\plrv[\data_1][\data_2][\mech_2] \geq \tau-s )   
-e^{\epsilon_2}P(\plrv[\data_2][\data_1][\mech_2] \leq -(\tau-s) )
\right)P(\plrv[\data_1][\data_2][\mech_1] = s)$$

This means that if for some $\tau$ and $c$ we have
$$c P(\plrv[\data_1][\data_2][\mech^*]>t)+ (1-c) P(\plrv[\data_1][\data_2][\mech^*]\geq t) 
- e^\epsilon\Big( c P(\plrv[\data_2][\data_1][\mech^*] < -t) +  (1-c) P(\plrv[\data_2][\data_1][\mech^*]\leq -t)\Big)>0$$

then there exists an $s\leq \epsilon_1$ for which 

$$c P(\plrv[\data_1][\data_2][\mech^*]>t)+ (1-c) P(\plrv[\data_1][\data_2][\mech^*]\geq t) 
- e^\epsilon\Big( c P(\plrv[\data_2][\data_1][\mech^*] < -t) +  (1-c) P(\plrv[\data_2][\data_1][\mech^*]\leq -t)\Big)>0$$


The case of $\delta_2=0$ is similar. Thus, without loss of generality, we can assume $\delta_1>0$ and $\delta_2>0$.


For $\mech_1$, pick the smallest $\tau_1$ and $c_1\in[0,1]$ such that $cP(\plrv[\data_1][\data_2][\mech]>\tau_1) + (1-c) P(\plrv[\data_1][\data_2][\mech]\geq \tau_1)=\delta_1$. Since $\mech_1$ satisfies $(\epsilon_1,\delta_1)$-\pbdp, this means that $cP(\plrv[\data_1][\data_2][\mech]>\tau_1) + (1-c) P(\plrv[\data_1][\data_2][\mech]\geq \tau_1) = e^\epsilon\Big( cP(\plrv[\data_2][\data_1][\mech]<-\tau_1) + (1-c) P(\plrv[\data_2][\data_1][\mech]\leq -\tau_1)\Big)$.


\end{proofEnd}

\end{comment}
